An Optimal Algorithm for Adversarial Bandits with Arbitrary Delays

We propose a new algorithm for adversarial multi-armed bandits with unrestricted delays. The algorithm is based on a novel hybrid regularizer applied in the Follow the Regularized Leader (FTRL) framework. It achieves $\mathcal{O}(\sqrt{kn}+\sqrt{D\log(k)})$ regret guarantee, where $k$ is the number of arms, $n$ is the number of rounds, and $D$ is the total delay. The result matches the lower bound within constants and requires no prior knowledge of $n$ or $D$. Additionally, we propose a refined tuning of the algorithm, which achieves $\mathcal{O}(\sqrt{kn}+\min_{S}|S|+\sqrt{D_{\bar S}\log(k)})$ regret guarantee, where $S$ is a set of rounds excluded from delay counting, $\bar S = [n]\setminus S$ are the counted rounds, and $D_{\bar S}$ is the total delay in the counted rounds. If the delays are highly unbalanced, the latter regret guarantee can be significantly tighter than the former. The result requires no advance knowledge of the delays and resolves an open problem of Thune et al. (2019). The new FTRL algorithm and its refined tuning are anytime and require no doubling, which resolves another open problem of Thune et al. (2019).

==> lower_bound_bob.tex <==

%\iffalse
\section{Lower bounds}
\resetnotes
\begin{algorithm}
\caption{Adversarial choice of $\ell$}
\label{alg:adv ell}
\DontPrintSemicolon
\KwIn{$x$}
\KwInit{$\cI=\{\argmax_ix_i\}$}
\LinesNumberedHidden
\While{$\sum_{i\in \cI}x_i + \min_{i\in\bar\cI}x_i\leq \frac{2}{3}$ }{
	Update $\cI \leftarrow \cI\cup \{\argmin_{i\in\bar\cI}x_i\}$	\;
}
\Return{ $\ell_i =\begin{cases}\min\{1,\frac{\sum_{i\in\bar\cI}x_i}{\sum_{i\in\cI}x_i}\} &\text{ for }i\in \cI\\
\max\{-1,-\frac{\sum_{i\in\cI}x_i}{\sum_{i\in\bar\cI}x_i}\}&\text{ for }i\in \bar\cI\end{cases}$}
\end{algorithm}

\begin{lemma}
\label{lem:variance of losses}
For any $x\in\Delta([k])$ such that $\max_ix_i\leq \frac{2}{3}$, the vector $\ell$ returned from \cref{alg:adv ell} satisfies
$\ell\in[-1,1]$, $\ip{x,\ell}=0$ and $\sum_{i=1}^k x_i\ell_i^2 \geq \frac{1}{2}$.
\end{lemma}
\begin{proof}
The first two properties follow directly from construction.
For the third property we bound the ratio of the two sets.
Assume $\sum_{i\in \cI}x_i<\frac{1}{3}$, then $\argmin_{i\in\bar\cI}x_i<\frac{1}{3}$ and the algorithm does not return yet.
Therefore we have $\frac{1}{3}\leq\sum_{i\in \cI}x_i\leq \frac{2}{3}$. Denote $p = \min\{\sum_{i\in \cI}x_i,\sum_{i\in \bar\cI}x_i\}$, we have just shown that $\frac{1}{3}\leq p$.
The quantity in question is therefore bounded by
\begin{align*}
\sum_{i=1}^k x_i\ell_i^2 = \sum_{i\in\cI} x_i\ell_i^2+\sum_{i\in\bar\cI} x_i\ell_i^2 = p + (1-p)\left(\frac{p}{1-p}\right)^2 = \frac{p}{1-p}\geq \frac{1}{2}\,.
\end{align*}
\end{proof}
\begin{claim}
\label{clm:exp lower bound}
For any $x\geq-\frac{1}{2}:\, \exp(x)-x-1 \geq \frac{x^2}{4}$.
\end{claim}
\begin{claim}
\label{clm:equality of bregman}
For any potential $F$ and $x\in\Delta([k])$, it holds that
\begin{align*}
D_{\overline{F}^*}(\nabla F(x)-\ell,\nabla F(x)) = \min_{c\in\R}D_{F^*}(\nabla F(x)-\ell+c\ones,\nabla F(x))\,.
\end{align*}
\end{claim}
\begin{claim}
\label{clm:negentropy}
For the negentropy potential $F(x)=\eta^{-1}\sum_{i=1}^k\log(x_i)x_i$, it holds that
\begin{align*}
-\overline F^*(-L) -\min_i L_i = \eta^{-1}\log(\max_i \nabla \overline F^*(-L)_i)\,. 
\end{align*}
\end{claim}
\begin{proof}
Denote $i^*=\argmin_{i\in[k]}L_i$. The negentropy has an explicit form of the constrained convex conjugate: $\overline F^*(-L) = \eta^{-1}\log(\sum_{i=1}^k\exp(-\eta L_i))$.
\begin{align*}
-\overline F^*(-L) -L_{i^*} &=  -\eta^{-1}\log\left(\sum_{i=1}^k\exp(-\eta L_i)\right) + \eta^{-1}\log(\exp(-\eta L_{i^*}))\\
&=-\eta^{-1}\log\left(\frac{\sum_{i=1}^k\exp(-\eta L_i)}{\exp(-\eta L_{i^*})}\right)=\eta^{-1}\log\left(\nabla \overline F^*(-L)_{i^*}\right)
\end{align*}
\end{proof}

\begin{theorem}\label{thm:full-info lower bound}
Let $(d_t)_{t=1}^n$ a sequence of positive reals and assume that
\begin{align*}
\max_{t\in[n]}d_t \leq \sqrt{\sum_{t=1}^nd_t^2/\log(k)}\,,
\end{align*}
then the minimax regret of the full information game in which the loss range of the adversary at round $t$ is limited to $d_t$ is lower bounded by
\begin{align*}
\Reg^*_n \geq \frac{1}{32}\sqrt{\sum_{t=1}^nd_t^2\log(k)}\,.
\end{align*}
If instead $n\leq \log(k)$ then the minimax regret is lower bounded by 
\begin{align*}
\Reg^*_n \geq \frac{1}{2}\sum_{t=1}^nd_t\,.
\end{align*}
\end{theorem}
\begin{proof}
We begin with the second statement.
Define an active set $\cA_1 = [k]$.
For any $t$, we randomly select half of the arms in $\cA_t$ to assign $\ell_{t,i} = -d_t/2$ and the other half $\ell_{t,i} = d_t/2$. (In case of an uneven number $|\cA_t|$ we leave one arm at $0$.) All other losses are $0$. We reduce $\cA_{t+1}=\{i\in\cA_t\,|\,\ell_{t,i}<0\}$ to the set of arms that were negative.
The set $\cA$ will not be empty since $\log(k) < \log_2(k)$, so the construction is valid. The expected loss of any player is always 0, while the loss of the best arm is 
$\min_{a}\sum_{t=1}^n\ell_{t,a}=-\sum_{t=1}^nd_t/2$, which concludes the second part of the theorem

We continue with the first part of the theorem.
Set $\eta = \sqrt{\log(k)/(\sum_{t=1}^nd_t^2)}$, $F(x) = \eta^{-1}\sum_{i=1}^k x\log(x)$ and
 $L_t = \sum_{s=1}^{t-1}\ell_t$.
For any given algorithm, let the adversary follow \cref{alg:adversary} for the selection of the losses.
Denote $\tau:=\argmax\{t\in[n+1]\,|\,\ell_{t-1} \neq 0\}$, then the regret of algorithm $\cA$ can be bounded as
\begin{align*}
\Reg_n(\cA) &= \sum_{t=1}^n \ip{x_t,\ell_t}-\min_{a^*\in\Delta([k])}\ip{a^*, L_{n+1}}\\
&\overset{\eqnote{
By construction $\ip{x_t,\ell_t}\geq 0 = \ip{z_t,\ell_t}$.
}}{\geq} \sum_{t=1}^n \ip{z_t,\ell_t}-\min_{a^*\in[k]}\ip{a^*,L_{n+1}}\\
&\overset{\eqnote{
Adding and subtracting the telescoping sum.
}}{=} \sum_{t=1}^n \left(\bar F^*(-L_{t+1})-\bar F^*(-L_{t})+\ip{z_t,\ell_t}\right)+\bar F^*(0)-\bar F^*(-L_{n+1})- \min_{a^*\in\Delta([k])}\ip{a^*,L_{n+1}}\\
&\overset{\eqnote{
follows from \cref{clm:shift,clm:gradient}.
}}{=} \sum_{t=1}^n D_{\bar F^*}(\nabla F(z_t)-\ell_t,\nabla F(z_t))+\eta^{-1}\log(k)-\bar F^*(-L_{\tau})- \min_{a^*\in\Delta([k])}\ip{a^*,L_{\tau}}\\
&\overset{\eqnote{
applies \cref{clm:equality of bregman,clm:negentropy}.
}}{=} \sum_{t=1}^n \min_{c\in\R}D_{F^*}(\nabla F(z_t)-\ell_t+c\ones,\nabla F(z_t))+\frac{\log(k)+\log(\max_{i\in[k]}z_{\tau,i})}{\eta}\\
&= \sum_{t=1}^n \left(\min_{c\in\R}\eta^{-1}\sum_{i=1}^kz_{t,i}\left(\exp(-\eta(\ell_{t,i}-c))-\eta (\ell_{t,i}- c) -1\right)\right)+\bbI\{\tau<n\}\frac{\log(k)+\log(2/3)}{\eta}\\
&\overset{\eqnote{
The $c^*=\argmin_c(...)$ is given by $c^*=\log(\sum_{i=1}^kz_i\exp(-\eta\ell_{t,i}))\leq -\eta \frac{d_t}{2}$, so we can apply \cref{clm:exp lower bound}.
}}{\geq} \sum_{t=1}^n \left(\min_{c\in\R}\eta\sum_{i=1}^k\frac{z_{t,i}}{4}(\ell_{t,i}- c)^2\right)+\bbI\{\tau\leq n\}\frac{2\log(k)}{5\eta}\\
&\geq \sum_{t=1}^n \eta\sum_{i=1}^k\frac{z_{t,i}}{4}\ell_{t,i}^2+\bbI\{\tau<n\}\frac{2}{5}\sqrt{\sum_{t=1}^nd^2\log(k)}\\
&\overset{\eqnote{
follows from \cref{lem:variance of losses}.
}}{\geq} \eta\frac{\sum_{t=1}^{\tau-1} d_t^2}{32}+\bbI\{\tau\leq n\}\frac{2}{5}\sqrt{\sum_{t=1}^nd^2\log(k)}\\
&\geq \frac{1}{32}\bbI\{\tau=n+1\}\sqrt{\sum_{t=1}^nd^2\log(k)}+\frac{2}{5}\bbI\{\tau\leq n\}\sqrt{\sum_{t=1}^nd^2\log(k)}\\
&\geq \frac{1}{32}\sqrt{\sum_{t=1}^nd^2\log(k)}
\end{align*}
\writeeqnotes
\end{proof}

\begin{theorem}
The minimax regret of the adversarial bandits with delay problem in which the adversary is restricted to a set of delays $(d_t)_{t=1}^n$ which he can use in arbitrary order is for sufficiently large $n$ bounded from below by
\begin{align*}
\Reg^* = \Omega\left(\max\{\sqrt{kn},\min_{S\subset[n]}|S|+\sqrt{D_{\bar S}\log(k)}\}\right)\,.
\end{align*}
\end{theorem}
\begin{proof}
Since the delay problem is strictly harder than the no delay problem, the general bandit lower bound of $\sqrt{kn}$ applies.
In the case that $\min_{S\subset[n]}|S|+\sqrt{D_{\bar S}\log(k)}$ is the dominating term, we reduce the problem to a full information game.
Lets first sort the set of delays in decreasing order, so assume that $d_1\geq d_2\geq \dots \geq d_n$.
Next we are putting the delays greedily into buckets such that an agent would need to make all decisions within a bucket without observing another entry. I.e. the first bucket is $\cB_1=\{1,2,\dots,b_1\}$ such that $b_1=\max\{t\in[n]\,|\,\forall\, s< t:\, s+d_s \geq t\}$. We iteratively define
$b_{m+1} = \max\{t\in[n]\,|\,\forall\, b_m<s<t:\,s+d_s\geq t\}$ and the $m+1$-th bucket goes from $\cB_{m+1}=\{b_m+1,b_m+2,\dots,b_{m+1}\}$.
If we set all losses within a bucket to the same value, then this problem is strictly harder then the full-information game with losses in range $|\cB_1|,|\cB_2|,\dots,$.
If the total number of buckets $M$ is smaller than $\log(k)$, we can directly apply \cref{thm:full-info lower bound} to get a lower bound of order $\Reg^*_n \geq \sum_{m=1}^M|\cB_m|/2=n/2\geq 1/2\min_{S\subset[n]}|S|+\sqrt{D_{\bar S}\log(k)}\}$.
Otherwise the total number of buckets $M$ is larger than $\log(k)$ and we permutate the delays in the range of the first $\log(k)$ buckets such that the first $\log(k)$ bucket sizes differ maximally by $1$ and call these new buckets $\tilde\cB$. (It is easy to see that this construction is possible, as long as the bucket sizes differ by at least 2, pick the first element of the larger bucket and put it into the smaller bucket.)
Now we are playing the full information game again.
We can directly apply \cref{thm:full-info lower bound} and obtain a lower bound of
\begin{align*}
\Reg^*_n \geq \frac{1}{32}\sqrt{\sum_{m=1}^{M}|\tilde\cB_m|^2\log(k)}\geq \frac{1}{32}\sqrt{(\sum_{m=1}^{\log(k)}|\cB_m|)^2+\sum_{m=\log(k)+1}^M|\cB_m|^2\log(k)}.
\end{align*}
Now we analysis how that term relates to the actual delay sequence.
First note that by construction of the buckets, it holds that $\forall\, t \in \cB_{m+1}:\,d_t\leq |\cB_m|$.
Assume that in bucket $\cB_m$ we have $d_{b_{m-1}+1}=\alpha_m$ and $d_{b_m}=\beta_m$ 
If this is the last bucket then we have $\sum_{t\in\cB_M}d_t-|\cB_M|^2\leq |\cB_M|\alpha_M-|\cB_M|^2\leq \frac{\alpha_M^2}{4}$.
Otherwise we have at least $\beta_m$ elements of delay $\beta_m$ (or the bucket would be bigger):
\begin{align*}
\sum_{t\in\cB_m}d_t-|\cB_m|^2 &\leq \beta_m^2 + (|\cB_m|-\beta_m)\alpha_m-|\cB_m|^2 \leq \begin{cases}
0 \mbox{ if }\beta_m \leq \frac{\alpha_m}{2} \\
(\beta_m-\alpha_m)\beta_m+\frac{\alpha_m^2}{4} \text{ if }\beta_m < \frac{\alpha_m}{2}
\end{cases}\\
&\leq \frac{\alpha_m^2}{4}-\frac{\beta_m^2}{4}\,.
\end{align*}
Since $\beta_m\geq\alpha_{m+1}$, we have
\begin{align*}
(\sum_{m=1}^{\log(k)}|\cB_m|)^2+\sum_{m=\log(k)+1}^M|\cB_m|^2\log(k) &\geq  |\cB_{\log(k)}|^2\log(k)^2+\sum_{t\in \cup_{m> \log(k)}\cB_m}d_t\log(k) - |\cB_{\log(k)}|^2\log(k)\\
&\geq \sum_{t\in \cup_{m> \log(k)}\cB_m}d_t\log(k)\,.
\end{align*}
Let $S' = \cup_{m\leq \log(k)}\cB_m$, we have shown that $\Reg^*_n =\Omega\left(|S'|\right)$ and $\Reg^*_n =\Omega\left(\sqrt{\sum_{t\in\bar{S}'}d_t\log(k)}\right)$ and therefore 
\begin{align*}
\Reg^* = \Omega\left(\max\{\sqrt{kn},\min_{S\subset[n]}|S|+\sqrt{D_{\bar S}\log(k)}\}\right)\,.
\end{align*}
\end{proof}

\begin{algorithm}
\caption{Adversary}
\label{alg:adversary}
\KwIn{Actor $\cA$, potential $\bar F^*$}
\DontPrintSemicolon
\LinesNumberedHidden
\For{$t= 1,\ldots,n$}{
	Set $z_t=\nabla \bar F^*(-L_t)$	\;
	\If{$\max_{i\in[k]}x_i> \frac{2}{3}$}{$\ell_t=0$\;}
	\Else{
	Get $\ell$ from \cref{alg:adv loss} with $x=z_t$.\;
	Determine $x_t = \cA((\ell_s)_{s=1}^{t-1})$\;
	Set $\ell_t = \operatorname{sign}(\ip{x_t,\ell})d_t\ell/2$\;
}
}
\end{algorithm}


\section{Stochastic Analysis}

We need to bound the second term by
\begin{align*}
\E\left[(2)\right]\leq \E\left[c\sum_{t=1}^n\sum_{i\neq i^*}x_{t,i}\eta_t\mathfrak{d}_t\right]\,,
\end{align*}
instead of 
\begin{align*}
\E\left[(2)\right]\leq \E\left[c\sum_{t=1}^n\eta_t\mathfrak{d}_t\right]\,,
\end{align*}
which we have proven before.
First note that if $x_{t,i^*} \leq \frac{1}{2}$, then 
\begin{align*}
\eta_t\mathfrak{d}_t \leq 2 (1-x_{t,i^*})\eta_t\mathfrak{d}_t\,.
\end{align*}
The next case is $\forall s\in\,\{s<t\,|\,d_s+s\geq t\}:\,x_{s,i^*} > \eta_t\mathfrak{d}_t$,
which implies $\hat L^{miss}_{ti^*}\leq \frac{1}{\eta}$.

Then we have 
\begin{align*}
&\overline F_t^*(-\hat L^{obs}_t)-\overline F_t^*(-\hat L^{obs}_t-\hat\ell_t)-\overline F_t^*(-\hat L^\rho_t)+\overline F_t^*(-\hat L^\rho_{t+1})\\
&\overset{\eqnote{
uses the Fundamental theorem of calculus together with the inequality above.
}}{\leq} \int_{0}^1 \ip{\hat\ell_t,\nabla \overline F_t^*(-\hat L^{obs}_t-x\hat\ell_t)}\,dx -\int_{0}^1 \ip{\hat\ell_t, \nabla\overline F^*_t(-\hat L^{obs}_t-\hat L^{miss}_{t,A_t}\e_{A_t} - x\hat\ell_t)}\,dx\\
&\overset{\eqnote{
substitutes $\tilde{z}(x) = \nabla \overline F_t^*(-\hat L^{obs}_t-x\hat\ell_t)$ and applies \cref{clm:gradient}.
}}{=} \int_{0}^1 \ip{\hat\ell_t,\tilde z(x)- \nabla\overline F^*_t(\nabla F_t(\tilde{z}(x))-\hat L^{miss}_{t,A_t}\e_{A_t})}\,dx\\
&\overset{\eqnote{
The probalities sum up to 1.
}}{=} \int_{0}^1 \ip{\hat\ell_{t,A_t}(\ones-\e_{A_t}),\nabla \overline F^*_t(\nabla F_t(\tilde{z}(x))-\hat L^{miss}_{t,A_t}(\e_{A_t}-\ones))-\tilde z(x)}\,dx\\
&\leq \int_{0}^1 \ip{\hat\ell_{t,A_t}(\ones-\e_{A_t}),\nabla F^*_t(\nabla F_t(\tilde{z}(x))-\hat L^{miss}_{t,A_t}(\e_{A_t}-\ones))-\tilde z(x)}\,dx\\
&= \sum_{i\neq A_t}\int_{0}^1 \hat\ell_{t,A_t}({f^*_t}'(f'_t(\tilde{z}_i(x))+\hat L^{miss}_{t,A_t})-\tilde z_i(x))\,dx\\
&\leq \sum_{i\neq A_t}\int_{0}^1 \hat\ell_{t,A_t}({f^*_{t2}}'(f'_{t2}(\tilde{z}_i(x))+\hat L^{miss}_{t,A_t})-\tilde z_i(x))\,dx\\
&= \int_{0}^1 \hat\ell_{t,A_t}(\tilde z_{A_t}(x)- {f^*}'_t(f'_t(\tilde{z}_{A_t}(x))-\hat L^{miss}_{t,A_t})\,dx\\
&\overset{\eqnote{
${f^*}'(t)$ is convex, so $-{f^*}'(f'(\tilde z_{A_t}) - \ell)\leq -\tilde z_{A_t} + {f^*}''(f'(\tilde z_{A_t}))$.
}}{\leq} \int_{0}^1 \hat\ell_{t,A_t}({f^*}''_t(f'_t(\tilde{z}_{A_t}(x)))\hat L^{miss}_{t,A_t}\,dx\\
&=\int_{0}^1 \ell_{t,A_t}x_{t,A_t}^{-1}f''_t(\tilde{z}_{A_t}(x))^{-1}\hat L^{miss}_{t,A_t}\,dx\\
&\overset{\eqnote{
follows because $\tilde z_{A_t}\leq x_{t,A_t}$ and $f_t''(x)^{-1}$ is monotonically increasing.
}}{\leq}\int_{0}^1 \ell_{t,A_t}x_{t,A_t}^{-1}f''_t(x_{t,A_t})^{-1}\hat L^{miss}_{t,A_t}\,dx\\
&\leq  x_{A_t}^{-1}f_{t2}''(x_{A_t})^{-1}\hat L^{miss}_{t,A_t}\\
& = \eta_t\hat L^{miss}_{t,A_t}\,.
\end{align*}
\writeeqnotes
Finally due to the unbiasedness of the loss estimators we have in expectation
\begin{align*}
\E[\hat L^{miss}_{t,A_t}] = \sum_{s:\rho(s)<\rho(t)}\bbI\{s+d_s\geq t\}\ell_{s,A_t} \leq \mathfrak{d}^\rho_t\,.
\end{align*}


We define $\tilde x_t := \nabla \bar F_t^*(-\hat L^\rho_t)$. 
\begin{lemma}
	For any $x\in(0,1)$, and positive $y>0$, the function
 \[{f_t^*}'(f_t'(x)-y) \]
is concave and the function 
 \[{f_t^*}'(f_t'(x)+y) \]
if convex for $x\in(0,(f_t^*)'(-y))$.
\end{lemma}
\begin{proof}
First we calculate the second derivative:
\begin{align*}
\left({f_t^*}'(f_t'(x)+z)\right)'' = \left({f_t^*}''(f_t'(x)+z)f_t''(x)\right)'=\left(\frac{f_t''(x)}{f_t''({f_t^*}'(f_t'(x)+z))}\right)'\\
= \frac{f_t'''(x)f_t''({f_t^*}'(f_t'(x)+z))-f_t''(x)f_t'''({f_t^*}'(f_t'(x)+z)){f_t^*}''(f_t'(x)+z)f_t''(z)}{f_t''({f_t^*}'(f_t'(x)+z))^2}=\frac{f_t'''(x)f_t''(\tilde x)-f_t'''(\tilde x) \frac{f_t''(x)^2}{f_t''(\tilde x)}}{f_t''(\tilde x)^2}
\end{align*}
Therefore the function is locally convex if $f_t'''(x)f_t''(\tilde x)^2 - f_t'''(\tilde x)f_t''(x)^2 > 0$ and concave otherwise.
We can explicitly calculate the quantities:
\begin{align*}
f_t'''(x)f_t''(\tilde x)^2 - f_t'''(\tilde x)f_t''(x)^2 \\= -(\frac{3}{4}\sqrt{t}x^{-\frac{5}{2}}+\eta_t^{-1}x^{-2})(\frac{1}{2}\sqrt{t}{\tilde x}^{-\frac{3}{2}}+\eta_t^{-1}{\tilde x}^{-1})^2+(\frac{3}{4}\sqrt{t}{\tilde x}^{-\frac{5}{2}}+\eta_t^{-1}{\tilde x}^{-2})(\frac{1}{2}\sqrt{t}{x}^{-\frac{3}{2}}+\eta_t^{-1}{x}^{-1})^2\\
={\tilde x}^{-\frac{3}{2}}x^{-\frac{3}{2}}\left((\frac{3}{4}\sqrt{t}+\eta_t^{-1}{\tilde x}^\frac{1}{2})(\frac{t}{4}x^{-\frac{1}{2}}+\sqrt{t}\eta_t^{-1}+\eta_t^{-2}x^{\frac{1}{2}})-(\frac{3}{4}\sqrt{t}+\eta_t^{-1}{x}^\frac{1}{2})(\frac{t}{4}{\tilde x}^{-\frac{1}{2}}+\sqrt{t}\eta_t^{-1}+\eta_t^{-2}{\tilde x}^{\frac{1}{2}}) \right) \\
={\tilde x}^{-\frac{3}{2}}x^{-\frac{3}{2}}\left(\frac{3t^\frac{3}{2}}{16}(x^{-\frac{1}{2}}-{\tilde x}^{-\frac{1}{2}})+\frac{3}{4}\sqrt{t}\eta_t^{-2}(x^\frac{1}{2}-{\tilde x}^\frac{1}{2})+\frac{t}{4}\eta_t^{-1}({\tilde x}^\frac{1}{2}x^{-\frac{1}{2}}-x^\frac{1}{2}{\tilde x}^{-\frac{1}{2}})+\sqrt{t}\eta_t^{-2}({\tilde x}^{\frac{1}{2}}-x^\frac{1}{2})\right)\\
={\tilde x}^{-\frac{3}{2}}x^{-\frac{3}{2}}\left(\frac{3t^\frac{3}{2}}{16}x^{-\frac{1}{2}}{\tilde x}^{-\frac{1}{2}}({\tilde x}^{\frac{1}{2}}-x^{\frac{1}{2}})+\frac{t}{4}\eta_t^{-1}x^{-\frac{1}{2}}{\tilde x}^{-\frac{1}{2}}({\tilde x}-x)+\frac{\sqrt{t}}{4}\eta_t^{-2}({\tilde x}^{\frac{1}{2}}-x^\frac{1}{2})\right)
\end{align*}
Therefore if $\tilde x = {f^*}'(f'(x)+z) < x$, then the function is concave and otherwise convex. 
The proof is completed by noting that ${f^*}'(f'(x)+z) < x\, \Leftrightarrow\, z <0$.
\end{proof}
%\fi

\newpage
\section{Open Problem}
Reminder: 
\begin{align*}
x_t = \nabla \overline F_t^*(-\hat L^{obs}_t)\,,\qquad\tilde x_t = \nabla \overline F_t^*(-\hat L^\rho_t)\,.\\
F_t(x) = \sum_{i=1}^k \frac{-2}{\sqrt{t}}\sqrt{x_i}+\eta_t^{-1}x_i\log(x_i)\,\\
\E\left[\hat L^{miss}_t\right]=\E\left[\hat L^{rho}_t-\hat L^{obs}_t\right] \leq \eta_t^{-1}\,. 
\end{align*}
The stochastic analysis uses the self-bounding proof of \cite{ZS19}, which bounds the regret by 
\begin{align*}
\E\left[\sum_{t=1}^T\sum_{i\neq i^*} 2\frac{\sqrt{x_{t,i}}}{\sqrt{t}}-\Delta_i x_{t,i}\right]\,.
\end{align*}
In the bandit with delay problem, the terms $\tilde x_t$ and $x_t$ are not identical, so we have instead:
\begin{align*}
\E\left[\sum_{t=1}^T\sum_{i\neq i^*} \frac{\sqrt{x_{t,i}}}{\sqrt{t}}+\frac{\sqrt{\tilde x_{t,i}}}{\sqrt{t}}-\Delta_i x_{t,i}\right]\,.
\end{align*}
In order to use our normal self-bounding proof, we need to replace
$\Delta_i x_{t,i}$ by $\frac{\Delta_i}{2}( x_{t,i}+\tilde x_{t,i})$.

This implies that we need to bound
\begin{align*}
\E\left[\sum_{t=1}^T\sum_{i\neq i^*}\Delta_i(\tilde x_{t,i}-x_{t,i})\right]\,.
\end{align*}
It seems very unlikely that this term is actually positive, since $\tilde x_{t,i}$ contains more information than $x_{t,i}$, but it is surprisingly hard to prove.

\paragraph{Constant delays:} One setting in which I can get a satisfactory bound is when all delays are constant $d$. In that case $x_{t+d}$ and $\tilde x_{t}$ are calculated based on the same loss estimators, but with different learning rates. I can show that $\min\{\tilde x_{t,i},1/k\} \leq x_{t+d,i}$, which can be used in the self bounding proof with some additional effort.

\paragraph{General setting:} We can make the problem easier by trying to prove 
\begin{align*}
\E\left[\sum_{t=1}^T\sum_{i\neq i^*}\Delta_i(\tilde x_{t,i}-ex_{t,i})\right] \leq 0\,.
\end{align*}
(This will suffice and increase the total regret by a small factor. $e$ can be replaced by any small problem independent factor)

If all $\Delta_i$ are identical, then I can prove the stronger statement
\begin{align*}
\E\left[\ip{\Delta,\tilde x_t} \,\middle|\,x_t\right]-e\ip{\Delta,x_t}\leq 0\,. 
\end{align*}

If the potential would only consist of the negentropy part, then I can even prove
\begin{align*}
\forall i:\,\E[\tilde x_{t,i} \,|\,x_t] - e x_{t,i}\leq 0\,.
\end{align*}

\begin{proof}
if $x_{t,i} \geq \frac{1}{e}$, then the statement is trivial. Otherwise 
\begin{align*}
\tilde x_{t,i} &= \frac{x_{t,i}\exp(-\eta_t\hat L^{miss}_{t,i})}{\sum_{j=1}^kx_{t,j}\exp(-\eta_t\hat L^{miss}_{t,j})}\\
&\leq \frac{x_{t,i}}{x_{t,i}+\sum_{j\neq i}x_{t,j}\exp(-\eta_t\hat L^{miss}_{t,j})}\\
&\leq \frac{x_{t,i}}{x_{t,i}+(1-x_{t,i})\exp(-\eta_t\sum_{j\neq i}\frac{x_{t,j}}{1-x_{t,i}}\hat L^{miss}_{t,j})}
\end{align*}
Denote $L = \sum_{j\neq i}\frac{x_{t,j}}{1-x_{t,i}}\hat L^{miss}_{t,j}$, then this is a random variable with mean $\E[L]\leq \eta_t^{-1}$.

It remains to show that given a positive random variable $L$ with mean bounded by $\eta_t^{-1}$ and any $x < \frac{1}{e}$, it holds that
\begin{align*}
\E\left[\frac{x}{x+(1-x)\exp(-\eta_t L)}\right] \leq e x\,.
\end{align*}
This can be seen by showing that for $x\leq 1/e$, the LHS is concave and we can pull the expectation inside.
\end{proof}

Unfortunately, the proof does not hold anymore for our actual potential and I am unable to reduce the problem to the negentropy case.



==> rebuttal.tex <==
We would like to thank all reviewers for their feedback.

1)
There is currently no lower bound for the unbounded setting. We believe that an adaptation of the lower bound of Cesa-bianchi et al (2016) is possible if the adversary is allowed to permutate the delays arbitrarily (but is not allowed to change the ``balanceness''). The problem can then be reduced to a full information game with varying loss intervals $[0,b_t]$. To our best knowledge, there does not exist any lower bound for that problem either. When using the standard approach for full information lower bounds, i.e. considering i.i.d. losses for all arms, it becomes significantly harder to quantify the shape of the cumulated loss distributions.
 
We do not change $a_t$ of older timesteps. If at some point $l>t$ we deactivate $a_l$, it will not affect the past choice.

2) The sum works the following way:
Let $f(x) = 2sqrt(x)$, then  we have 
\begin{align*}
\sum_{t=1}^n \eta_t \mathfrak{d}_t&= \sqrt{\log(K)/2}\sum_{t=1}^n  \mathfrak{d}_tf'(\mathfrak{D}_t)\\
&\leq\sqrt{\log(K)/2}\sum_{t=1}^n \int_{\mathfrak{D}_{t-1}}^{\mathfrak{D}_t}f'(x)\dx \\
&= \sqrt{\log(K)/2}(f(\mathfrak{D}_n)-f(\mathfrak{D}_0))=\sqrt{2\log(K)\mathfrak{D}_n}.
\end{align*}
The $+1$ is indeed unneccesary.

3) There is no doubling trick known to turn the $\sqrt{log(K)(KT+D)}$ bound with known $T$ and $D$ into an anytime algorithm. A new paper published at NeurIPS this year (not public during submission of our paper) has managed to use doubling to obtain $\sqrt{\log(K)(K^2T+D)}$, which is suboptimal if $d<K^2\log(K)$. The difficiulty here is that we have to double according to two quantities T and D simultaneously. Regarding our second result for refined bounds in the unbalanced case: the existing algorithm by Thune et al already uses a doubling trick and still requires additional information.

As we mentioned, there is no known algorithm that obtains bounds close to us without extra information, therefore we don't think experiments are of interest.

We believe that our worst-case improvement is mainly in the analysis and could also be transfered to EXP3 based algorithms. However our regularizer closes the log(K) gap for small delay budgets and is also a promising candidate for algorithms that perform optimal in both the stochastic and adversarial setting.

###################
trimmed reviewer feedback

Questions
- I would have liked to see a full discussion of related work in the paper.
- I would also like to see more details on the algorithm of Thune et al. (2019) given here for comparison
- The authors say that their regret is rate optimal. Is there a lower bound for the problem where the delays can be arbitrary? If so, can this be added to the table of results. If not, what are the challenges in adapting the lower bound from Cesa-bianchi et al (2016?
- Regarding the advanced tuning, am I right in thinking that $\tilde D_t$ is an increasing function of t? So then, can it happen that $d_s>\sqrt{\tilde D_t/log(k)}$ for some $t$ but $d_s\leq\sqrt{\tilde D_l/log(k)}$ for some $l>t$? What would happen in this case? As the algorithm has already defined $a$ using $t$, would it have to be changed or would it stay the same?
- It may be good to have more details of the advanced tuning

Minor comments:
- The second paragraph of the introduction is very long. Breaking it up would make it easier to read
- Several references are lacking details of where the paper was published (e.g. Pogodin and Lattimore, 2019, Zimmert et al, 2019).
- I think the notation $\bar{S}$ is being used to denote the complementary set. It would be helpful to include this in the definitions section.




The proof of Theorem 1 seems to skip a step. Given the setting of eta_t, it is clear why eta_n^{-1} log k is equal to \sqrt{2 \mathfrak{D}_n log k}. However, can you explain further how you get that \sum_{t=1}^n \eta_t \mathfrak{d}_t <= \sqrt{2 \mathfrak{D}_n log k} ? If not in the main text, then explaining it in the supplementary material would be helpful. It seems vaguely familiar from the analysis of another online learning algorithm.

In the second part of Theorem 1, why do you have sqrt{8(D+1) log k} instead of sqrt{8 D log k} ? The proof suggests the latter.


It is not clear why simply using the doubling trick for the unknown D and n and without forgetting the data obtained up to a doubling episode (similarly to how doubling trick is used for MDP by UCRL2 which extends trivially to MAB) would not lead to a good solution. It should also be an anytime algorithm.

Given that the theoretical improvement in the bound is very small (sqrt (log k) together with the fact that the D term and the D free term are in two separate Sqrt ) experiments should have been performed with Thune et al algorithm (possibly with doubling trick as used by UCRL2 i.ie without resetting the data) to validate the improvement. And check if the improvement is due to a loose analysis in Thune et al results or if it is due to a real algorithmic-improvement.

The paper should clearly define what they mean by anytime algorithm (for ex if it means to guarantee a good regret whp for any time step n)
3. [Score] Please provide an overall score for the submission.
Accept: Good paper
4. [Questions for the Authors] Please provide questions for authors to address during the author feedback period and point out which improvement would improve your score.
I would like the authors to address my concerns regarding the weaknesses identified in section 2.

Anytime algorithm definition

Is the improvement due to a better algorithm or a looser analysis in Thune et al algorithms? 



